Multivariate predictions of local reduced-order-model errors and dimensions

This paper introduces multivariate input-output models to predict the errors and bases dimensions of local parametric Proper Orthogonal Decomposition reduced-order models. We refer to these multivariate mappings as the MP-LROM models. We employ Gaussian Processes and Artificial Neural Networks to construct approximations of these multivariate mappings. Numerical results with a viscous Burgers model illustrate the performance and potential of the machine learning based regression MP-LROM models to approximate the characteristics of parametric local reduced-order models. The predicted reduced-order models errors are compared against the multi-fidelity correction and reduced order model error surrogates methods predictions, whereas the predicted reduced-order dimensions are tested against the standard method based on the spectrum of snapshots matrix. Since the MP-LROM models incorporate more features and elements to construct the probabilistic mappings they achieve more accurate results. However, for high-dimensional parametric spaces, the MP-LROM models might suffer from the curse of dimensionality. Scalability challenges of MP-LROM models and the feasible ways of addressing them are also discussed in this study.

==> Parameter_range_2.tex <==
%----------------------------------------------------------------------------------------------------------------------
\subsection{Applications of MP-LROM error prediction models}
\subsubsection{Designing the decomposition of the parametric domain}
\label{sec:parametric_map}
%----------------------------------------------------------------------------------------------------------------------

We seek to build a decomposition of the viscosity domain $[0.01,1]$  for the 1D-Burgers model using the MP-LROM models introduced in Section \ref{sect:err_estimate}. The non-physical parameter $\nu$ is set to $1$. As discussed in Section \ref{sect:problem_Des}, we take the following steps. First we identify ``$\mu_p$-feasible'' intervals $[d_\ell,d_r]$  in the parameter space such that local reduced-order model depending only on the high-fidelity trajectory at $\mu_p$ is accurate to within the prescribed threshold for any $\mu \in [d_\ell,d_r]$. Second, a greedy algorithm generates the decomposition
%
\begin{equation}
  [0.01,1] \subset \bigcup_{i=1}^M\, \left[d_\ell^i,d_r^i\right],
\end{equation}
%
by covering the parameter space with a union of $\mu_{p_i}$ feasible intervals, where each $\mu_{p_i}$-feasible interval is characterized by an error threshold $\bar \varepsilon_i$ (which can vary from one interval to another). This relaxation is suggested since for intervals associated with small parameters $\mu_{p_i}$, it is difficult to achieve small reduced-order models errors similar to those obtained for larger parametric configurations.

For the existing reduced basis methods a global reduced-order model depending on multiple high-fidelity trajectories is usually constructed. In contrast, our approach uses the MP-LROM models to decompose the parameter space into smaller regions where the local reduced-order model solutions are {\color{red}accurate to within }some  tolerance levels. Since the local bases required for the construction of the local reduced-order models depend on only a single full simulation, the {\color{red}dimension} of the {\color{red}POD subspace} is small, leading to lower on-line computational complexity.
%-----------------------------------------------------------------------------------------------------------------------
\setcounter{secnumdepth}{5}
\paragraph{Construction of a $\mu_p-$feasible interval}
\label{sec:feasible_interval}
%-----------------------------------------------------------------------------------------------------------------------
 We noticed in the previous subsection that MP-LROM models can accurately estimate $\log \varepsilon_{\mu,\mu_p,K_{POD}}^{HF}$ \eqref{eqn:param_rang_err} associated with reduced-order models. Thus we can employ them to establish a range of viscosity parameters around $\mu_p$ such that the reduced-order solutions depending on $U_{\mu_p}$ satisfy some desired accuracy level. More precisely, starting from parameter $\mu_p$, a fixed POD basis dimension and a tolerance error $\log\bar{\varepsilon}$, we are searching for an interval $[d_l, d_r]$ such that the estimated prediction $\widehat{\log\varepsilon}_{\mu,\mu_p,K_{POD}}^{HF}$ of the true error $\log\varepsilon_{\mu,\mu_p,K_{POD}}^{HF}$ \eqref{eqn:param_rang_err} meets the requirement
\begin{equation}\label{eqn:inequality_constraint}
 \widehat{\log\varepsilon}_{\mu,\mu_p,K_{POD}}^{HF}<\log\bar{\varepsilon}, \forall \mu \in [d_l, d_r].
\end{equation}

Our proposed strategy makes use of a simply incremental approach by sampling the vicinity of $\mu_p$ to account for the estimated errors $\widehat{\log\varepsilon}_{\mu,\mu_p,K_{POD}}^{HF}$  forecasted by the MP-LROM models defined before. A grid of new parameters $\mu$ is built around $\mu_p$ and the error models predict the errors outward of $\mu_p$. Once the error models outputs are larger than the prescribed error $\log\bar{\varepsilon},$ the previous $\mu$ satisfying the constraint \eqref{eqn:inequality_constraint} is set as $d_l$, for $\mu < \mu_p$ or  $d_r$ for $\mu > \mu_p$.



Figure \ref{fig:expm2_range} illustrates the range of parameters predicted by the MP-LROM models via ANN and GP against the true feasible interval and the results show good agreement. For this experiment we set ${\mu_p}=0.7$, dimension of {\color{blue}POD subspace} $K_{POD} = 9$ and $\bar{\varepsilon} = 10^{-2}$.  Values of $\mu = \mu_p \pm 0.001\cdot i,$ $i=1,2,\ldots$ are passed to the MP-LROM models. The average range of parameters obtained over five different configurations with ANN is $[0.650, 0.780]$ while in the case of GP we obtained $[0.655,0.780]$.
In each configuration, we train the model with $80 \%$ random split of the data set and test it over the fixed test set of Figure \ref{fig:expm2_range}. For this design, the true range of parameters is $[0.650,0.785]$ underlying the predicting potential of MP-LROM models built using the regression machine learning techniques.


%
%\begin{center}
\begin{figure}[H]
	\begin{centering}
	\includegraphics[width=0.5\textwidth, height=0.40\textwidth]{truth_error_compare.eps}
   \caption{The average range of parameter $\mu$ obtained with MP-LROM {\color{blue}models} for $K_{POD}=9$ and ${\mu_p}=0.7$. The desired accuracy is $\bar{\varepsilon} = 10^{-2}$. The numbers represent the left and the right edges of the predicted vs the true feasible intervals.} \label{fig:expm2_range}	
	\end{centering}
\end{figure}
%\end{center}
%

%----------------------------------------------------------------------------------------------------------------------------
\paragraph{The decomposition of the parametric domain as a union of $\mu_p-$feasible intervals}
\label{sec:parametric_map}
%----------------------------------------------------------------------------------------------------------------------------

A union of different $\mu_{p_k}$-feasible intervals can be designed to cover a general entire 1D-parametric domain $[A,B]$. Once such construction is {\color{red} available, it} will allow for reduced-order simulations with a-priori error quantification for any value of viscosity parameter $\mu \in [A,B]$.

A greedy strategy based on the MP-LROM error models constructed in {\color{red} Section} \ref{sect:err_estimate} is described in Algorithm \ref{alg:map_generation} and its output is a collection of feasible intervals $\cup_{k=1}^n[d_l^k,d_r^k] \supset [A,B]$. After each iteration $k$ of the algorithm, a $\mu_{p_k}$-feasible interval $[d_l^k,d_r^k]$ is constructed. Each interval is associated with some accuracy threshold $\bar{\varepsilon}_k$.  For small viscous parametric values we found out that designing $\mu_{p_k}-$feasible intervals associated with higher precision levels (very small thresholds $\bar{\varepsilon}_k$) is impossible since the dynamics of parametric 1D-Burgers model solutions change dramatically with smaller viscosity parameters.
In consequence we decided to let $\bar{\varepsilon}_k$ vary along the parametric domain to accommodate the solution physical behaviour. Thus a small threshold $\bar{\varepsilon}_0$ will be initially set and as we will advance charting the parameter domain $[A,B]$ from right to left, the threshold $\bar{\varepsilon}_k$ will be increased.

The algorithm starts by selecting the first centered parameter $\mu_{p_0}$ responsible for basis generation. It can be set to $\mu_{p_0} = B$ but may take any value in the proximity of $B$,~$\mu_{p_0}\leq B$. This choice depends on the variability of parametric solutions in this domain region and by selecting $\mu_{p_0}$ to differ from the right edge of the domain, the number $n$ of the feasible intervals should decrease.

The next step is to set the threshold $\bar{\varepsilon}_0$ along with the maximum permitted size of the initial feasible interval to be constructed. This is set to $2\cdot r_0$, thus $r_0$ can be referred as the interval radius. Along with the radius, the parameter $\Delta r$ will decide the maximum number of MP-LROM model calls employed for the construction of the first $\mu_{p_0}$-feasible interval. While the radius is allowed to vary during the algorithm iterations, $\Delta r$ is kept constant. Finally the dimension of POD basis has to be selected together with three parameters $\beta_1,~\beta_2$ and $\beta_3$ responsible for changes in the threshold and radius and selecting a new parameter location $\mu_{p_k}$ encountered during the procedure.

Next the algorithm starts the construction of the $\mu_{p_0}$ feasible interval. The process is described in the top part of Figure \ref{fig:describe_algorithm}(a). Then we are sampling the vicinity of $\mu_{p_0}$ for equally distributed parameters $\mu$ and compute the MP-LROM model predictions. The sampling process and the comparison between the predicted errors $\widehat{\log{{\varepsilon}}}_{\mu,\mu_{p_0},K_{POD}}^{HF}$ and $\log\bar{\varepsilon}_0$ are depicted in Figure \ref{fig:describe_algorithm}(a). A green vertical segment indicates that the estimated error satisfies the threshold; i.e., $\widehat{\log{{\varepsilon}}}_{\mu,\mu_{p_0},K_{POD}}^{HF} < \log\bar{\varepsilon}_0$, whereas the red segment indicates the opposite. The left limit of the $\mu_{p_0}-$feasible
interval is obtained when either $\mu > \mu_{p_0}-r_0$ or $\widehat{\log{{\varepsilon}}}_{\mu,\mu_{p_0},K_{POD}}^{HF}> \log{\bar{\varepsilon}_0}$. The left limit $d_l^0$, denoted with a green dashed line in Figure \ref{fig:describe_algorithm}(a), is set equal to the last parameter $\mu$ such that $\widehat{\log{{\varepsilon}}}_{\mu,\mu_{p_0},K_{POD}}^{HF} \leq \log{\bar{\varepsilon}_0}$.

The next step searches for a centered parameter $\mu_{p_{k+1}}$ and this process is described at the bottom of the Figure \ref{fig:describe_algorithm}(a) for $k=0$. The centered parameter $\mu_{p_{k+1}}$ is first proposed based on an empirical formula described in line $25$ of Algorithm \ref{alg:map_generation}. This formula depends on the current centered parameter $\mu_{p_k}$, the number of tested parameters $\mu$ during the construction of $\mu_{p_k}-$feasible interval, parameters $\Delta r$ and $\beta_3$. Next, the algorithm checks if the following constraint is satisfied

%\begin{equation}\label{eq::constrain1}
% [d_l^{k+1},d_r^{k+1}] \not \subset \bigg( \bigcup_{i=1}^{k} [d_l^{i},d_r^{i}] \bigg),
%\end{equation}

\begin{equation}\label{eq::constrain2}
 [d_l^{k+1},d_r^{k+1}] \bigcap \bigg( \bigcup_{i=1}^{k} [d_l^{i},d_r^{i}] \bigg) \neq \emptyset,
\end{equation}
without taking into account the MP-LROM model error. This is achieved by comparing the error model prediction $\widehat{\log{{\varepsilon}}}_{d_l^k,\mu_{p_{k+1},K_{POD}}}^{HF}$
and threshold $\log \bar{\varepsilon}_{k+1}$ (see instruction $27$ and bottom of Figure \ref{fig:describe_algorithm}(a) for $k=0$). If the predicted error is smaller than the current threshold, assuming a monotonically increasing error with larger distances $d(\mu,\mu_{p_{k+1}})$, the reduced-order model solutions should satisfy the accuracy threshold for all $\mu \in [\mu_{p_{k+1}},d_l^k].$ In consequence the equation \eqref{eq::constrain2} will be satisfied for the current $\mu_{p_{k+1}}$, if we set $r_{k+1}=\mu_{p_{k+1}}-d_l^k$ (see instruction $30$). In the case the error estimate is larger than the present threshold, the centered parameter $\mu_{p_{k+1}}$ is updated to the middle point between old $\mu_{p_{k+1}}$ and $d_l^k$ (see also the bottom of Figure \ref{fig:describe_algorithm}(a)). For the situation where the monotonic property of the error does not hold in practice, a simply safety net is used at instruction $12$.



The instructions between lines $5$ and $21$ generate the $\mu_{p_k}$-feasible interval, for the case when the current centered parameter $\mu_{p_k} \neq d_{l}^{k-1}$ (see top part of Figure \ref{fig:describe_algorithm}(b) for $k=1$). {\color{red} Here by {\it int} we refer to the integer part of a real number. We used the Matlab command floor for the implementation}. {\color{red} For situation when $\mu_{p_k} = d_l^{k-1}$ (see bottom of Figure \ref{fig:describe_algorithm}(b) for $k=2$), the threshold has to be increased (by setting $\bar{\varepsilon}_{k} = \beta_1\bar{\varepsilon}_k$ at line $23$), since the reduced-order model solutions can not satisfy the desired precision according to the predicted errors. {\color{red} In consequence, $\beta_1$ has to be selected larger than $1$. The need for relaxing the threshold suggests that the greedy search is currently operating into a parametric region where only a slight change in the parameter $\mu$ away from $\mu_{p_k}$ leads to predicted ROM errors larger than the current threshold. Relaxing the threshold and decreasing the radius size $(\textrm{select }\beta_2<1 \textrm{ in line 23 of Algorithm 3})$ can be used as a strategy to identify a feasible region for the current centered parameter $\mu_{p_k}$. Similarly, relaxing the threshold and expanding the search $(\beta_2>1)$ could also represent a viable strategy. However, expanding the search in a parametric regime with large changes in the model dynamics, even if the threshold was relaxed, may lead to useless evaluations of the expressions in lines $7$ and $18$ of the Algorithm 3. Thus $\beta_2$ should be selected smaller than $1$. Once the feasible region is obtained, the radius $r_k$ is reset to  the initial value $r_0$ (see line 25 of the Algorithm 3). By selecting $\beta_3 > 1$, the computational complexity of Algorithm $3$ is decreased since the first proposal of the new centered parameter $\mu_{p_{k+1}}$ will always be smaller than the left limit $d_l^k$ of the current feasible interval. The entire algorithm stops when $\mu_{p_{k+1}} \leq A.$}}


For our experiments we employed the ANN MP-LROM model, and we set $A=0.01$, $B=1$, $\bar{\varepsilon}_0 = { \color{blue} 10^{-2},~\Delta r = 5 \times 10^{-3}},~r_0=0.5,~{K_{POD}} = 9,~\beta_1 = 1.2,~\beta_2 = 0.9$ and $\beta_3=1.4$.  We initiate the algorithm by setting $\mu_{p_0}=0.87$, and the first feasible interval $[ 0.7700,1]$ is obtained. Next the algorithm selects $\mu_1=0.73$ with the associated range of $[ 0.6700,0.8250]$ using the same initial threshold level. As we cover the parametric domain from right to left; i.e., selecting smaller and smaller parameters $\mu_{p_k}$, the algorithm enlarges the current threshold $\bar{\varepsilon}_k$, otherwise the error model predictions would not satisfy the initial precision. We continue this process until we get the threshold $6.25$ with $\mu_{32}=0.021$ and the corresponding feasible interval $[0.01,0.039]$. The generated decomposition is depicted in Figure \ref{fig:expm2_numMus} where the associated threshold varies with the parameter change.


%
\begin{algorithm}
 \begin{algorithmic}[1]
% \Algphase{START}
\State Select $\mu_{p_0}$ as the right edge of the parameter interval, i.e. $\mu_{p_0} = B$.
\State Set error threshold $\hat{\varepsilon}_0$, step size $\Delta r$ for selection of sampling parameters $\mu$, the maximum search radius $r_0$, dimension of POD basis $K_{POD}$ and $\beta_1,~\beta_2$ and $\beta_3$.
\State Set $k=0$.
\State WHILE $\mu_{p_k} \geq A$ Do
 \State $\quad$ FOR {\color{red}$i=1$} to $int(\frac{r_k}{\Delta r})+1$
 \State $\quad \quad$  Set $\mu = \mu_{p_k} + i \Delta r$
  \State $\quad \quad$  IF $(\phi(\mu,\mu_{p_k},{K_{POD}}) > \log\bar{\varepsilon}_k ~{\color{red}\textrm{OR}~\mu>B)}$  THEN
  \State $\quad \quad \quad$  Set $d_r^k = \mu_{p_k} + (i-1) \Delta r$. EXIT.
 \State $\quad \quad$  END IF
 \State $\quad$END FOR
 \State $\quad$IF $k>0$ THEN
    \State $\quad \quad$  IF $d_r^k<d_l^{k-1}$ THEN
      \State  $\quad \quad \quad$ $\mu_{p_k} = \frac{\mu_{p_k}+d_l^{k-1}}{2}$. GOTO $5$.
    \State $\quad \quad$END IF
  \State $\quad$END IF
\State $\quad$FOR $j=1$ to $int(\frac{r_k}{\Delta r})+1$
  \State  $\quad \quad$  Set $\mu = \mu_{p_k} - j \Delta r$
  \State $\quad \quad$  IF $(\phi(\mu,\mu_{p_k},{K_{POD}}) > \log\bar{\varepsilon}_k ~{\color{red}\textrm{OR}~\mu<A})$  THEN
  \State $\quad \quad \quad$ Set $d_l^k = \mu_{p_k} - (j-1) \Delta r$. EXIT.
  \State $\quad \quad$  END IF
   \State $\quad$END FOR
\State $\quad$IF {\color{red}$(i=1)$}.OR.{\color{red}$(j=1)$} THEN
\State $\quad \quad$  Set $\bar{\varepsilon}_{k} = \beta_1 \cdot \bar{\varepsilon}_k$; $r_{k} = \beta_2 \cdot r_k$;  GOTO $5$.
\State $\quad$ELSE
\State $\quad \quad$  $\mu_{p_{k+1}} = \mu_{p_k} - \beta_3 (j-1) \Delta r$; $\bar{\varepsilon}_{k+1} = \bar{\varepsilon}_k$; ${\color{red} r_{k+1} = r_0}.$
\State $\quad$END IF
\State $\quad $WHILE $\phi(d_l^k,\mu_{p_{k+1}},{K_{POD}}) > \log\bar{\varepsilon}_{k+1}$ DO
\State $\quad \quad$  $\mu_{p_{k+1}} = \frac{\mu_{p_{k+1}} + d_l^k}{2}$.
\State $\quad$END WHILE
\State $\quad$ Set $r_{k+1}=\mu_{p_{k+1}}-d_l^k$.
\State $\quad$ $k=k+1$.
\State END WHILE
 %THEN STOP.
\end{algorithmic}
 \caption{\color{red} Generation of 1D-parametric domain decomposition for reduced-order models usage. Extension to multi-dimensional parametric space is subject to future research.}
 \label{alg:map_generation}
\end{algorithm}



%
\begin{figure}[h]
  \begin{centering}
  \subfigure[Designing the first feasible interval (1) and selecting a new centered  \newline parameter $\mu_{p_1}$ (2)] {\includegraphics[trim={4.6cm 0.5cm 0.0cm 1cm},scale=0.3]{Alg_photoa.pdf}}
  \subfigure[Designing a feasible interval (3) and increasing the tolerance level (4) ]
 {\includegraphics[trim={4.6cm 0.5cm 2.7cm 1cm},scale=0.3]{Alg_photob.pdf}}
\caption {{\color{red} A description of the most important stages of the parameter domain decomposition algorithm.  The arrows describe the internal steps for each stage initiated in the order depicted by the arrows' indices. }}
\label{fig:describe_algorithm}
  \end{centering}
\end{figure}
%
%\begin{center}
\begin{figure}[H]
	\begin{centering}
	\includegraphics[width=0.5\textwidth, height=0.40\textwidth]{range_plot.pdf}
    \caption{The diffusion parametric domain decomposition defining the local feasible intervals and their corresponding errors. Associated with one feasible interval there is a centered parameter $\mu_p$ high-fidelity trajectory that guides the construction of a reduced basis and operators such that the subsequent reduced-order model solutions along this interval are accurate to within the threshold depicted by the Y-axis labels.}
	\label{fig:expm2_numMus}
	\end{centering}
\end{figure}

%\end{center}
%
%-------------------------------------------------------------------------------------------------------------------------

